Retrieval & Fine-Tuning for In-Context Tabular Models

Tabular data is a pervasive modality spanning a wide range of domains, and the inherent diversity poses a considerable challenge for deep learning. Recent advancements using transformer-based in-context learning have shown promise on smaller and less complex datasets, but have struggled to scale to larger and more complex ones. To address this limitation, we propose a combination of retrieval and fine-tuning: we can adapt the transformer to a local subset of the data by collecting nearest neighbours, and then perform task-specific fine-tuning with this retrieved set of neighbours in context. Using TabPFN as the base model -- currently the best tabular in-context learner -- and applying our retrieval and fine-tuning scheme on top results in what we call a locally-calibrated PFN, or LoCalPFN. We conduct extensive evaluation on 95 datasets curated by TabZilla from OpenML, upon which we establish a new state-of-the-art with LoCalPFN -- even with respect to tuned tree-based models. Notably, we show a significant boost in performance compared to the base in-context model, demonstrating the efficacy of our approach and advancing the frontier of deep learning in tabular data.

==> content/ideas.tex <==

{\color{gray}
\section{Some ideas and arguments: not an actual section}
\begin{itemize}
    \item Local vs global information: Tree based models are really good at splitting the space into independent chunks: NN don't do that and try to fit a big function for everything
    \item While this is great for some modalities (images etc) it is not for tabular data \url{https://arxiv.org/abs/2207.08815}
    \item Local methods such as kNN and kernel methods are well-known ways to construct classifiers based on local information
    \item Transformers/ICL fundamentally are similar to kernel methods. Especially TabPFN whose main architectural insight is to transpose the transformer and make it attend on different datapoints instead of different features.
    \item We can leverage than in TabPFN by giving more importance to closer points instead of all points
    \item \ac{We want to compare against TabR, we should be much faster (and maybe better)}
    \item \rasa{For local vas global: We can argue finetune is gradient based
update on full dataset and then cite this \citep{von2023transformers} and 
say kNN is doing a local version of finetuning for each point.(the paper is for regression)}
\end{itemize}
}

==> content/related2.tex <==
\section{Related Work}

\subsection{Deep Learning for Tabular Data}

Recent advancements in deep learning for tabular data have introduced various novel approaches. TabR \cite{gorishniy2024tabr} proposes a retrieval-augmented model with an empirically-tuned retrieval block inspired by kNN, incorporating similarity and value modules. While it lacks comprehensive experiments, TabR's MLP-like backbone may be less expressive than the transformer-based TabPFN.

TuneTables \cite{feuer2024tunetables} optimizes PFNs through prompt-tuning, compressing large datasets into smaller contexts for multi-objective optimization and enhanced interpretability. Despite addressing dataset size scalability through data summarization techniques, TuneTables struggles with feature set scalability and excessive memory consumption without significant gains.

SAINT \cite{somepalli2022saint} improves neural networks for tabular data using row attention and contrastive pre-training, employing self-attention blocks for columns and rows. Its reliance on balanced datasets with binary classes and lack of in-context learning limit its applicability.

Differential nearest neighbours regression (DNNR) \cite{nader2022dnnr} proposes techniques to make kNN differentiable, showcasing the potential of simple methods like kNN in different forms, although it tackles a separate scope from our method.

\subsection{Retrieval-Augmented and Fine-Tuning Methods}

Fine-Tuning the Retrieval Mechanism for Tabular Deep Learning \cite{breejen2023exploring} emphasizes tailoring retrieval processes to enhance model performance. TabPFGen \cite{ma2023tabpfgen} and Distill \cite{ma2024context} integrate retrieval and generative techniques, proposing innovative methods for improved performance.

An Inductive Bias for Tabular Deep Learning \cite{beyazit2024inductive} discusses leveraging domain-specific knowledge to design effective tabular deep learning models. The work "Why do tree-based models still outperform deep learning on typical tabular data" \cite{grinsztajn2022tree} examines the persistent superiority of tree-based models over deep learning approaches.

Interpretable Machine Learning for TabPFN \cite{rundel2024interpretable} enhances the interpretability of TabPFN models, making predictions more understandable. Retrieval \& Interaction Machine for Tabular Data Prediction \cite{qin2021retrieval} and Self-Attention Between Datapoints \cite{kossen2021selfattention} introduce non-parametric deep learning models that leverage retrieval and interaction mechanisms, although NPT's reliance on the entire training dataset as context can be a limitation.

\subsection{General Notes}

Several recent attempts to build tabular deep learning models through retrieval-augmented approaches have emerged \cite{gorishniy2024tabr, somepalli2022saint}. The nearest neighbors technique remains a fundamental yet actively explored algorithm \cite{nader2022dnnr}. Retrieval methods are also widely used in other domains, such as Natural Language Processing (NLP) and computer vision, highlighting their cross-disciplinary applicability.


